EAGLE: Large-scale Vehicle Detection Dataset in Real-World Scenarios using Aerial Imagery

Multi-class vehicle detection from airborne imagery with orientation estimation is an important task in the near and remote vision domains with applications in traffic monitoring and disaster management. In the last decade, we have witnessed significant progress in object detection in ground imagery, but it is still in its infancy in airborne imagery, mostly due to the scarcity of diverse and large-scale datasets. Despite being a useful tool for different applications, current airborne datasets only partially reflect the challenges of real-world scenarios. To address this issue, we introduce EAGLE (oriEnted vehicle detection using Aerial imaGery in real-worLd scEnarios), a large-scale dataset for multi-class vehicle detection with object orientation information in aerial imagery. It features high-resolution aerial images composed of different real-world situations with a wide variety of camera sensor, resolution, flight altitude, weather, illumination, haze, shadow, time, city, country, occlusion, and camera angle. The annotation was done by airborne imagery experts with small- and large-vehicle classes. EAGLE contains 215,986 instances annotated with oriented bounding boxes defined by four points and orientation, making it by far the largest dataset to date in this task. It also supports researches on the haze and shadow removal as well as super-resolution and in-painting applications. We define three tasks: detection by (1) horizontal bounding boxes, (2) rotated bounding boxes, and (3) oriented bounding boxes. We carried out several experiments to evaluate several state-of-the-art methods in object detection on our dataset to form a baseline. Experiments show that the EAGLE dataset accurately reflects real-world situations and correspondingly challenging applications.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/abstract.tex <==
\begin{abstract}
Multi-class-oriented vehicle detection from airborne imagery is a crucial task in the computer and remote vision domains. In the last decade, we have witnessed significant progress in object detection in ground imagery, but it is still in its infancy in airborne imagery, mostly due to the scarcity of diverse and large-scale datasets. Despite being a useful tool for different applications, current airborne datasets only partially reflect the challenges of real-world scenarios. Therefore, we introduce EAGLE (oriEnted object detection using Aerial imaGery in real-worLd scEnarios), a large-scale dataset for multi-class vehicle detection with object orientation information. It features aerial images of size \SI{5616x3744}{\px} composed of different real-world situations with a wide variety of flight altitude, weather, illumination, time, city, and camera positions. The annotation was done by airborne imagery experts with two main vehicle classes reflecting real-world situations. The large-scale EAGLE contains more than 215,000 instances annotated with oriented bounding boxes defined by four points and orientation, making it the largest dataset to date in this task. We define three tasks: detection by (1) horizontal bounding boxes, (2) rotated bounding boxes, and (3) oriented bounding boxes. We carried out several experiments to evaluate several state-of-the-art methods in object detection on our dataset to form a baseline. Experiments show that the EAGLE dataset accurately reflects real-world situations and correspondingly challenging applications.
%The dataset will be made publicly available.
\end{abstract}


==> sections/annotation.tex <==

\section{Annotation of\gls{EAGLE}}
\subsection{Images collection}
In airborne data, the image properties such as the resolution, time of capture, and sensor angle can create dataset biases.
To address this issue, we have collected the images from several different resolutions, capturing time, viewing angles and different commercially available camera sensors.
To even more enhance the data diversity, the images are captured from multiple regions, cities, and countries suitable for real-world scenarios such as flood, wildfire, earthquake, and search and rescue missions and so on.
The images contain the precise geographical information such as the location coordinate, and time of capture leading to no duplicity in the images.

\subsection{Category selection}
Considering the real-world applications and usability of object categories, the experts in the domain of aerial imagery interpretation have chosen two main vehicles in our\gls{EAGLE} dataset, including car and truck.
Unlike several existing datasets, \eg~\cite{cheng2016learning,zhu2015orientation,mundhenk2016large}, we split the vehicle class into car and truck instead of only vehicle due to their different appearances and effects on the traffic flow. These two classes are the main traffic participants.
In ~\ref{fig:comparedatasets in vehicle}, to compare\gls{EAGLE} with other datasets which currently have the largest number of vehicle annotations, we provide a comparison with DOTA~\cite{Xia2017DOTA} and NWPU VHR10~\cite{cheng2016learning}.
It can be noted that\gls{EAGLE} surpasses these recent datasets by a large margin. 

\subsection{Annotation method}
We consider different ways of annotating. In computer vision, many visual concepts such as region descriptions,objects, attributes, and relationships, are annotated with bounding boxes, as shown in [12]. A common description of bounding boxes is (xc, yc, w, h), where (xc, yc) is the center location,w, hare the width and height of the bounding box, respectively. Objects without many orientations can be adequately annotated with this method. However, bounding boxes labeled in this way cannot accurately or compactly outline oriented instances such as text and objects in aerial images. In an extreme but actually common condition as shown in Fig.3(c) and (d), the overlap between two bounding boxes is so large that state-of-the-art object detection methods cannot differentiate them. In order to remedy this, we need to find annotation method suitable for oriented objects.An option for annotating oriented objects isθbased oriented bounding box which is adopted in some text detection benchmarks [37], namely (xc, yc, w, h, θ), whereθdenotes the angle from the horizontal direction of the standard bounding box. A flaw of this method is the inability to compactly enclose oriented objects with large deformation among different parts. Considering the complicated scenes and various orientations of objects in aerial images,we need to abandon this method and choose a more flexible and easy to understand way. An alternative is arbitrary quadrilateral bounding boxes, which can be denoted as{(xi, yi), i= 1,2,3,4}, where(xi, yi) denotes the positions of the oriented bounding boxes’ vertices in the image.The vertices are arranged in a clockwise order. This way is widely adopted in oriented text detection benchmarks [11].We draw inspiration from these researches and use arbitrary quadrilateral bounding boxes to annotate objects.To make a more detailed annotation, as shown in Fig.3,we emphasize the importance of the first point(x1, y1),which normally implies the “head” of the object. For helicopter, large vehicle, small vehicle, harbor, baseball diamond, ship and plane, we carefully denote their first point to enrich potential usages. While for soccer field, swimming pool, bridge, ground track field, basketball court and tennis court, there are no visual clues to decide the first point, so we choose the top left point as the starting point.Some samples of annotated patches (not the whole original image) in our dataset are shown in Fig.4.It is worth noticing that, Papadopoulos et al.[23] have explored an alternative annotation method and verify its efficiency and robustness. We assume that the annotations would be more precise and robust with more elaborately designed annotation methods, and alternative annotation protocols would facilitate more efficient crowd-sourced image annotations.

\subsection{Dataset splits}
In order to ensure that the training data and test data distributions approximately match, we randomly select half of the original images as the training set, 1/6 as validation set,and 1/3 as the testing set. %We will publicly provide all the original images with ground truth for training set and validation set, but not for the testing set. For testing, we are currently building an evaluation server.


==> sections/motivation.tex <==

\section{Motivation}
Datasets have played an important role in data driven research in recent years [36,6,14,40,38,33]. Large datasets like MSCOCO ~\cite{Lin2014} are instrumental in promoting object detection and image captioning research. When it comes to the classification task and scene recognition task, the same is true for ImageNet [6] and Places [40], respectively. However, in aerial object detection, a dataset resembling MSCOCO and ImageNet both in terms of image number and detailed annotations has been missing, which becomes one of the main obstacles to the research in Earth Vision, especially for developing deep learning based algorithms. Aerial object detection is extremely helpful for remote object tracking and unmanned driving. Therefore, a large scale and challenging aerial object detection benchmark, being as close as possible to real world applications, is imperative for promoting research in this field. We argue that a good aerial image dataset should possess four properties, namely, 1) a large number of images, 2)many instances per categories, 3) properly oriented object annotation, and 4) many different classes of objects, which make it approach to real world applications. However, existing aerial image datasets [41,18,16,25] share in common several shortcomings: insufficient data and classes, lack of detailed annotations, as well as low image resolution. Moreover, their complexity is inadequate to be considered as a reflection of the real world. Datasets like TAS [9], VEDAI [25], COWC [21]and DLR 3K Munich Vehicle [16] only focus on vehicles. UCASAOD [41] contains vehicles and planes while HRSC2016 [18] only contains ships even though fine grained category information are given. All these datasets are short in the number of classes, which restricts their applicability to complicated scenes. In contrast, NWPUVHR10 [2] is composed of ten different classes of objects while its total number of instances is only around3000. Detailed comparisons of these existing datasets are shown in Tab.1. Compared to these aerial datasets, as we shall see in Section 4,\gls{EAGLE} is challenging for its tremendous object instances, arbitrary but well distributed orientations, various categories and complicated aerial scenes. Moreover, scenes in\gls{EAGLE} is in coincidence with natural scenes, so\gls{EAGLE} is more helpful for real world applications.

\begin{table*}
    \begin{center}
    \caption{Comparison among EAGLE and object detection datasets in aerial images. BB is short for bounding box. One-dot refers to annotations with only the center coordinates of an instance provided. Fine-grained categories are not taken into account. For example, EAGLE consists of 2 different categories, but with extra difficult flags with respect to the class and orientation.}
        %\vspace{0.2cm}
    \resizebox{0.7\textwidth}{!}{
         \begin{tabular}{c|cccccc}
         %\toprule
         \hline
         Datasets & Categories & Images & Instances & Image (px) & Annotation 
         %& GSD(cm/pixel) 
         %& Aerial Coverage(km$^2$) 
         &Year\\
         \hline
         TAS~\cite{}&  1 & 30 & 1,310 & 792 & HBB & 2008 \\
         SZTAKI‐INRIA~\cite{}& 2 & 9 & 665 & ~800 & OBB & 2012 \\
         NWPUVHR‐10~\cite{} & 10 & 800 & 3775 & ~1000 & HBB & 2014 \\
         VEDAI~\cite{} & 9 & 1,210 & 3640 & 1024 & OBB & 2015 \\
         UCAS‐AOD~\cite{} & 2 & 910 & 6029 & 1280 & HBB & 2015 \\
         DLR3KVehicle~\cite{} & 2 & 20 & 14235 & 5616 & OBB & 2015 \\
         HRSC2016~\cite{} & 1 & 1,070 & 2976  & ~1000 & OBB & 2016 \\
         RSOD~\cite{} & 4 & 976 & 6950  & ~1000 & HBB & 2017 \\
         DOTA~\cite{} & 15 & 2806 & 188282 & 800-4000 & OBB & 2017\\
         %\midrule
         \hline
         EAGLE(ours) & 2 & 321 & 215,986 & 5616 & OBB & 2019\\
         %\bottomrule
         \hline
         \end{tabular}
         }
    \label{tab:stats}
   \end{center}
%    \vspace{-0.5cm}
\end{table*}


When it comes to general objects datasets, ImageNet and MSCOCO are favored due to the large number of images, many categories and detailed annotations. ImageNet has the largest number of images among all object detection datasets. However, the average number of instances per image is far smaller than MS COCO and our\gls{EAGLE}, plus the limitations of its clean backgrounds and carefully selected scenes. Images in\gls{EAGLE} contain an extremely large number of object instances, some of which have more than 1,000 instances. PASCAL VOC Dataset [7] is similar to ImageNet in instances per image and scenes but the inadequate number of images makes it unsuitable to handle most detection needs. Our\gls{EAGLE} resembles MSCOCO in terms of the instance numbers and scene types, but\gls{EAGLE}’s categories are not as many as MSCOCO because objects which can be seen clearly in aerial images are quite limited. Besides, what makes\gls{EAGLE} unique among the above mentioned large scale general object detection benchmark sis that the objects in\gls{EAGLE} are annotated with properly oriented bounding boxes(OBB for short). OBB can better enclose the objects and differentiate crowded objects from each other. The benefits of annotating objects in aerial images with OBB are further described in Section3. We draw a comparison among\gls{EAGLE}, PASCAL VOC, ImageNet and MSCOCO to show the differences in Tab.2.


\begin{table}
    %\begin{center}
    \caption{Comparison among\gls{EAGLE} and other general object detection datasets. BBox is short for bounding boxes, Avg. BBox quantity indicates average bounding box quantity per image. Note that for the average number of instances per image, \gls{EAGLE} surpasses other datasets hugely.}
        %\vspace{0.2cm}
    \resizebox{0.5\textwidth}{!}{
         \begin{tabular}{c|cccccc}
         %\toprule
         \hline
         Datasets & Category & #Image & #BBox  & Avg. #BBox \\
         \hline
        \multirow{2}{*}{PASCAL VOC ~\cite{}\\ (07++12)&  2021&50362&1992.89 }\\
         MS-COCO(2014 trainval)~\cite{}& 80123&287&886&2667.19 \\
         ImageNet(2017train)~\cite{} & 200&349&319&478&8061.37 \\
         \hline
        \gls{EAGLE}(ours) &2&2&806188&28267.10\\
         %\bottomrule
         \hline
         \end{tabular}
         }
    \label{tab:stats}
%    \end{center}
%    \vspace{-0.5cm}
\end{table}


==> sections/properties.tex <==
\section{Properties of\gls{EAGLE}}

\subsection{Image size}
Aerial images are usually very large in size compared to those in natural images dataset. The original size of images in our dataset ranges from about800×800to about4k×4k while most images in regular datasets (e.g. PASCALVOC and MSCOCO) are no more than1k×1k. We make annotations on the original full image without partitioning it into pieces to avoid the cases where a single instance is partitioned into different pieces.

\subsection{Various orientations of instances}
As shown in Fig.1(f), our dataset achieves a good balance in the instances of different directions, which is significantly helpful for learning a robust detector. Moreover, our dataset is closer to real scenes because it is common to see objects in all kinds of orientations in the real world.3977
(a)(b)(c)(d) Figure 3: Visualization of adopted annotation method. The yellow point represents the starting point, which refers to: (a) top left corner of a plane, (b) the center of sector shaped baseball diamond, (c) top left corner of a large vehicle. (d) is a failure case of the horizontal rectangle annotation, which brings high overlap compared to (c).Figure 4: Samples of annotated images in\gls{EAGLE}. We show three samples per each category, except six for large vehicle. (a)(b)(c) Figure 5: Statistics of instances in\gls{EAGLE}. AR denotes the aspect ratio. (a) The AR of horizontal bounding box. (b) The AR of oriented bounding box. (c) Histogram of number of annotated instances per image.3978

\subsection{Spatial resolution information}
We also provide the spatial resolution for each image in our dataset, which implies the actual size of an instance and plays a significant role in aerial object detection. The importance of spatial resolution for detection task are two folds. First, it allows the model to be more adaptive and robust for varieties of objects of the same category. It’s known that objects appear smaller when seen from a distance. The same object with different sizes will trouble the model and hurt classification. However, a model can pay more attention to the shape with resolution information provided instead of objects’ size. Second, it’s better for fine grained classification. For example, it will be simple to distinguish a small boat from a large warship. Spatial resolution can also be used to filter mislabeled outliers in our dataset, as intra-class varieties of actual sizes for most categories are limited. Outliers can be found by selecting the objects whose size is far different from those of the same category in a small range of spatial resolution.

\subsection{Various pixel size of categories}
Following the convention in [35], we refer to the height of a horizontal bounding box, which we call pixel size for short, as a measurement for instance size. We divide all the instances in our dataset into three splits according to their height of horizontal bounding box: small for range from10to50, middle for range from50to300, and large for range above300. Tab.3illustrates the percentages of three instance splits in different datasets. It is clear that the PASCAL VOC dataset, NWPU VHR10 dataset and DLR 3KMunich Vehicle dataset are dominated by middle instances, middle instances and small instances, respectively. However, we achieve a good balance between small instances and middle instances, which is more similar to real-world scenes and thus, helpful to better capture different size of objects in practical applications. It’s worth noting that pixel size varies in different categories. For example, a vehicle may be as small as30, however, a bridge can be as large as1200, which is 40$\times$ larger than a vehicle. The huge differences among instances from different categories make the detection task more challenging because models have to be flexible enough to handle extremely tiny and huge objects. Dataset 1050 pixel 50300 pixel above 300 pixel PASCAL VOC0.140.610.25MSCOCO0.430.490.08NWPU VHR100.150.830.02DLR 3K Munich Vehicle0.930.070\gls{EAGLE}0.570.410.02Table 3: Comparison of instance size distribution of some datasets in aerial images and natural images.

\subsection{Various aspect ratio of instances}
Aspect ratio (AR) is an essential factor for anchor-based models, such as Faster RCNN [27] and YOLOv2 [26]. We count two kinds of AR for all the instances in our dataset to provide a reference for better model design: 1) AR of minimally circumscribed horizontal rectangle bounding box, 2)AR of original quadrangle bounding box. Fig.5 illustrates these two types of distribution of aspect ratio for instances in our dataset. We can see that instances varies greatly in aspect ratio. Moreover, there are a large number of instances with a large aspect ratio in our dataset.

\subsection{Various instance density of images}
It is common for aerial images to contain thousands of instances, which is different from natural images. For example, images in ImageNet [6] contain on the average 2categories and 2 instances, while MSCOCO contains 3.5categories and 7.7 instances, respectively. Our dataset is much richer in instances per image, which can be up to2000. Fig.5illustrates the number of instances in our\gls{EAGLE} dataset.With so many instances in a single image, it is unavoidable to see areas densely crowded with instances. ForCOCO, instances are not annotated one by one because occlusion makes it difficult to distinguish an instance from its neighboring instances. In these cases, the group of instances is marked as one segment with attribute named “crowd”.However, this is not the case for aerial images because there are rarely occlusion due to the perspective from the above.Therefore, we can annotate all the instances in a dense area one by one. Fig.4shows examples of densely packed instances. Detecting objects in these cases poses an enormous challenge for the current detection methods.


